{\mu}-Bench: A Vision-Language Benchmark for Microscopy Understanding

Recent advances in microscopy have enabled the rapid generation of terabytes of image data in cell biology and biomedical research. Vision-language models (VLMs) offer a promising solution for large-scale biological image analysis, enhancing researchers' efficiency, identifying new image biomarkers, and accelerating hypothesis generation and scientific discovery. However, there is a lack of standardized, diverse, and large-scale vision-language benchmarks to evaluate VLMs' perception and cognition capabilities in biological image understanding. To address this gap, we introduce {\mu}-Bench, an expert-curated benchmark encompassing 22 biomedical tasks across various scientific disciplines (biology, pathology), microscopy modalities (electron, fluorescence, light), scales (subcellular, cellular, tissue), and organisms in both normal and abnormal states. We evaluate state-of-the-art biomedical, pathology, and general VLMs on {\mu}-Bench and find that: i) current models struggle on all categories, even for basic tasks such as distinguishing microscopy modalities; ii) current specialist models fine-tuned on biomedical data often perform worse than generalist models; iii) fine-tuning in specific microscopy domains can cause catastrophic forgetting, eroding prior biomedical knowledge encoded in their base model. iv) weight interpolation between fine-tuned and pre-trained models offers one solution to forgetting and improves general performance across biomedical tasks. We release {\mu}-Bench under a permissive license to accelerate the research and development of microscopy foundation models.

==> tables/classification_0.tex <==
\begin{tabular}{llllllll}
\toprule
Quartile & ALIGN & BLIP & BioMedCLIP & ConchCLIP & OpenCLIP & PLIP & QuiltCLIP \\
\midrule
(28, 37] & 0.26 (0.44) & 0.19 (0.39) & 0.34 (0.48) & 0.22 (0.42) & 0.22 (0.42) & 0.38 (0.49) & 0.23 (0.42) \\
(37, 62] & 0.13 (0.33) & 0.23 (0.42) & 0.21 (0.41) & 0.26 (0.44) & 0.25 (0.43) & 0.16 (0.36) & 0.27 (0.45) \\
(62, 68] & 0.3 (0.46) & 0.25 (0.43) & 0.32 (0.47) & 0.22 (0.41) & 0.28 (0.45) & 0.15 (0.36) & 0.16 (0.37) \\
(68, 81] & 0.31 (0.46) & 0.26 (0.44) & 0.25 (0.43) & 0.09 (0.28) & 0.32 (0.47) & 0.24 (0.43) & 0.18 (0.38) \\
\bottomrule
\end{tabular}


==> tables/cog_eval.tex <==
\begin{table}[!tb]
\setlength\tabcolsep{6pt}
\renewcommand{\arraystretch}{1.1}
\centering
\small
\begin{tabular}{ll}
\toprule
Model &  Acc $\uparrow$\\
\midrule
CogVLM &  \\
QwenVLM &  \\
\midrule
Random & 25.0 \\
\bottomrule
\end{tabular}
\caption{Evaluation of different VLMs on the cognitive dataset.}
\label{tab:cog_results}
\end{table}












% \begin{table}[!tb]
% \setlength\tabcolsep{6pt}
% \renewcommand{\arraystretch}{1.1}
% \centering
% \small
% \begin{tabular}{lllllll}
% \toprule
% Model &  Domain $\uparrow$& Modality $\uparrow$ & Stain $\uparrow$& Subdomain $\uparrow$& Submodality $\uparrow$ & Total $\uparrow$\\
% \midrule
% \midrule
% \textbf{Embedding}  \\  

% ALIGN  &  \\
% BLIP  &  \\
% OpenCLIP  &  \\ \\

% BioMedCLIP & \\
% QuiltCLIP &  \\
% PLIP &  \\
% ConchCLIP &  \\



% \midrule
% \textbf{Auto-Regressive} \\
% CogVLM &  \\
% QwenVLM &  \\

% \midrule
% \midrule
% Random &  \\
% \bottomrule
% \end{tabular}
% \caption{Evaluation of different VLMs on the cognitive dataset.}
% \label{tab:cog_results}
% \end{table}


==> tables/dataset_components.tex <==


\begin{table*}[t]
\centering
\normalsize
\renewcommand{\arraystretch}{1.25} 
\caption{Dataset Composition: Subdivision of each component of BIOVLM dataset (elements in * are not yet included)}
\begin{tabular}{m{2cm}m{4cm}m{7cm}m{2cm}m{2cm}}
\toprule
\textbf{Category} & \textbf{Task} & \textbf{Task Description} &  \textbf{Output} & \textbf{Metrics}  \\
\midrule

\textbf{Vision \& Language}   \\
\multirow{8}{5em}{Perception} & Structure Identification & Identify objects/structures (e.g., nuclei, mitochondria) & Text &  Precision, Recall, F1-score \\
& Modality Identification & Determine image modality (e.g. Brightfield, Fluorescence, Electron Microscopy) & Text & Accuracy, F1 score \\ 
 &  Magnification Assessment & Identify magnification level used  & Numeric &  MAE \\
& Biological System Categorization & Classify the biological system under study (e.g., immune cells, neurons) & Text & Accuracy, F1 score \\

& Fluorescence/Color Analysis & Evaluate signal intensity or color markers & Text& Quantitative measures, Sensitivity \\ 

& Size Measurement & Measure size of specific objects/structures in pixels or other units & Numeric &  MAE \\ 

& Counting and Quantification & Count number of cells, organelles, or other structures & Numeric & Mean absolute error\\
\\

   & Text-image segmentation & Create context sensitive masks from textual description & Image & IoU, dice coefficient  \\


\hline

\multirow{3}{5em}{Cognition}   & Image Quality Assessment &  Identify artifacts like fluorescence bleed-through & Text &  Sensitivity, Specificity \\

& Positional Reasoning Tasks & Describe position/location of objects/structures & Text &MAE or other measurement (bounding boxes, centroid, etc.) \\

& Attribute description  & Describe other attributes like texture or shape & Text & Accuracy  \\


  & *Contextual Understanding & Relate objects/structures to broader 
biomedical research context & Text & NLP-based metrics (e.g., BLEU for textual description)  \\ 



& *Image Contrast &  Compare and contrast images (what are difference between two images?) & Text & Accuracy, BLUE, BertScore\\

& *Visual Question Answering & Answer knoweldege intesnive questions based on image text pairs & Text & Accuracy, BLUE, BertScore\\




\midrule

\textbf{Language} \\
linguistic understanding   \\
Commonsense knowledge     \\
Biomedical Understanding     & Link prediction & Predict interaction of two elements across different spatial structures & Text & Accuracy \\








\bottomrule
\end{tabular}
\label{tab:category_analysis}
\end{table*}

==> tables/eval_classification.tex <==
\renewcommand{\arraystretch}{1}
\begin{adjustbox}{center}
\begin{tabular}{l{0.5cm}lllllll}

\toprule
 Classify: & ALIGN & BLIP & BioMedCLIP & ConchCLIP & OpenCLIP & PLIP & QuiltCLIP \\
\midrule
Cell contour & 0.3 (0.46) & 0.29 (0.46) & 0.29 (0.46) & 0.43 (0.5) & 0.35 (0.48) & 0.44 (0.5) & 0.39 (0.49) \\
Cell cycle phase (bf) & 0.08 (0.27) & 0.2 (0.4) & 0.15 (0.36) & 0.12 (0.33) & 0.3 (0.46) & 0.19 (0.39) & 0.04 (0.2) \\
Cell cycle phase (df) & 0.1 (0.3) & 0.2 (0.4) & 0.29 (0.46) & 0.02 (0.14) & 0.39 (0.49) & 0.1 (0.3) & 0.19 (0.39) \\
Cell cycle phase (ef) & 0.14 (0.35) & 0.34 (0.48) & 0.4 (0.49) & 0.36 (0.48) & 0.26 (0.44) & 0.26 (0.44) & 0.09 (0.29) \\
Cell eccentricity & 0.42 (0.5) & 0.3 (0.46) & 0.33 (0.47) & 0.4 (0.49) & 0.41 (0.49) & 0.44 (0.5) & 0.25 (0.44) \\
Cell texture & 0.36 (0.48) & 0.39 (0.49) & 0.41 (0.49) & 0.29 (0.46) & 0.36 (0.48) & 0.38 (0.49) & 0.2 (0.4) \\
Colocalization patterns & 0.23 (0.42) & 0.23 (0.42) & 0.27 (0.45) & 0.27 (0.45) & 0.08 (0.28) & 0.27 (0.45) & 0.15 (0.36) \\
Pollen & 0.52 (0.5) & 0.28 (0.45) & 0.05 (0.22) & 0.48 (0.5) & 0.1 (0.3) & 0.08 (0.27) & 0.23 (0.42) \\
Pre-cancerous and cervical cancer lesions & 0.24 (0.43) & 0.23 (0.42) & 0.14 (0.35) & 0.22 (0.42) & 0.52 (0.5) & 0.07 (0.26) & 0.43 (0.5) \\
Synhtetic White blood cell & 0.26 (0.44) & 0.17 (0.38) & 0.18 (0.39) & 0.12 (0.33) & 0.22 (0.42) & 0.13 (0.34) & 0.16 (0.37) \\
White blood cell & 0.18 (0.39) & 0.19 (0.39) & 0.14 (0.35) & 0.12 (0.33) & 0.16 (0.37) & 0.21 (0.41) & 0.21 (0.41) \\
amyloid beta morphology patterns (a) & 0.11 (0.31) & 0.29 (0.46) & 0.07 (0.26) & 0.92 (0.27) & 0.05 (0.22) & 0.03 (0.17) & 0.05 (0.22) \\
amyloid beta morphology patterns (b) & 0.26 (0.44) & 0.25 (0.44) & 0.45 (0.5) & 0.27 (0.45) & 0.18 (0.39) & 0.26 (0.44) & 0.31 (0.46) \\
clinical chronic heart failure & 0.53 (0.5) & 0.42 (0.5) & 0.68 (0.47) & 0.65 (0.48) & 0.56 (0.5) & 0.39 (0.49) & 0.37 (0.49) \\
colorectal cancer texture & 1.0 (0.0) & 0.08 (0.27) & 0.47 (0.5) & 0.9 (0.3) & 1.0 (0.0) & 0.77 (0.42) & 0.65 (0.48) \\
\bottomrule
\end{tabular}
\end{adjustbox}



==> tables/eval_old.tex <==
\begin{tabular}{lllllll}
\toprule
Model & Classification  $\uparrow$ & Domain $\uparrow$& Modality $\uparrow$& Subdomain $\uparrow$& Submodality $\uparrow$ & Total $\uparrow$\\
\midrule
\midrule
\textbf{Embedding}  \\  

Openclip & 0.105 (0.306) & 0.609 (0.488) & 0.03 (0.17) & 0.131 (0.337) & 0.001 (0.024) & 0.195 (0.397) \\ \\

Biomedclip & 0.103 (0.304) & 0.432 (0.495) & 0.793 (0.405) & 0.747 (0.435) & 0.71 (0.454) & 0.557 (0.497) \\
Plip & 0.137 (0.344) & 0.711 (0.453) & 0.177 (0.382) & 0.857 (0.35) & 0.063 (0.244) & 0.389 (0.488) \\

\midrule
\midrule
\textbf{Auto-Regressive} \\
\midrule
\midrule
Random & 0.195 (0.396) & 0.169 (0.375) & 0.251 (0.434) & 0.167 (0.373) & 0.17 (0.375) & 0.19 (0.393) \\
\bottomrule
\end{tabular}


==> tables/eval_small.tex <==
\begin{tabular}{lllllll}
\toprule
Model &  Domain $\uparrow$& Modality $\uparrow$ & Stain $\uparrow$& Subdomain $\uparrow$& Submodality $\uparrow$ & Total $\uparrow$\\
\midrule
\midrule
\textbf{Embedding}  \\  

ALIGN & 0.246 (0.431) & 0.026 (0.159) & 0.95 (0.219) & 0.393 (0.489) & 0.199 (0.4) & 0.229 (0.42) \\
BLIP & 0.155 (0.362) & 0.304 (0.46) & 0.15 (0.359) & 0.194 (0.396) & 0.125 (0.331) & 0.194 (0.396) \\
OpenCLIP & 0.212 (0.409) & 0.112 (0.316) & 0.06 (0.239) & 0.193 (0.395) & 0.047 (0.212) & 0.136 (0.343) \\ \\
BioMedCLIP & 0.079 (0.271) & 0.648 (0.478) & 0.46 (0.501) & 0.203 (0.403) & 0.268 (0.443) & 0.312 (0.463) \\
ConchCLIP & 0.409 (0.492) & 0.138 (0.345) & 0.05 (0.219) & 0.492 (0.5) & 0.101 (0.301) & 0.271 (0.444) \\
PLIP & 0.45 (0.498) & 0.498 (0.5) & 0.01 (0.1) & 0.628 (0.484) & 0.077 (0.266) & 0.397 (0.489) \\
QuiltCLIP & 0.141 (0.348) & 0.161 (0.368) & 0.21 (0.409) & 0.339 (0.474) & 0.114 (0.318) & 0.189 (0.392) \\

\midrule
\midrule
\textbf{Auto-Regressive} \\
CogVLM & 0.402 (0.491) & 0.578 (0.494) & 0.06 (0.239) & 0.649 (0.478) & 0.454 (0.498) & 0.506 (0.5) \\
QwenVLM & 0.597 (0.491) & 0.702 (0.457) & 0.04 (0.197) & 0.647 (0.478) & 0.326 (0.469) & 0.555 (0.497) \\

\midrule
\midrule
Random & 0.195 (0.396) & 0.169 (0.375) & 0.251 (0.434) & 0.167 (0.373) & 0.17 (0.375) & 0.19 (0.393) \\
\bottomrule
\end{tabular}


==> tables/eval_small_captions.tex <==
\begin{tabular}{lllllll}
\toprule
Model &  Domain $\uparrow$& Modality $\uparrow$ & Stain $\uparrow$& Subdomain $\uparrow$& Submodality $\uparrow$ & Total $\uparrow$\\
\midrule
\midrule
\textbf{Embedding}  \\  

ALIGN  & 0.43 (0.5) & 0.77 (0.42) & 0.37 (0.48) & 0.29 (0.45) & 0.46 (0.5) & 0.44 (0.5) \\
BLIP  & 0.21 (0.4) & 0.33 (0.47) & 0.22 (0.41) & 0.22 (0.42) & 0.19 (0.39) & 0.24 (0.43) \\
OpenCLIP  & 0.19 (0.39) & 0.81 (0.39) & 0.29 (0.45) & 0.37 (0.48) & 0.15 (0.36) & 0.36 (0.48) \\ \\

BioMedCLIP & 0.53 (0.5) & 0.8 (0.4) & 0.51 (0.5) & 0.59 (0.49) & 0.2 (0.4) & 0.49 (0.5) \\
QuiltCLIP & 0.13 (0.34) & 0.6 (0.49) & 0.41 (0.49) & 0.47 (0.5) & 0.24 (0.43) & 0.35 (0.48) \\
PLIP & 0.2 (0.4) & 0.64 (0.48) & 0.22 (0.41) & 0.5 (0.5) & 0.28 (0.45) & 0.35 (0.48) \\
ConchCLIP & 0.41 (0.49) & 0.26 (0.44) & 0.61 (0.49) & 0.5 (0.5) & 0.05 (0.21) & 0.37 (0.48) \\



\midrule
\textbf{Auto-Regressive} \\
CogVLM & 0.428 (0.495) & 0.59 (0.492) & 0.06 (0.239) & 0.677 (0.468) & 0.454 (0.498) & 0.525 (0.499) \\
QwenVLM & 0.597 (0.491) & 0.702 (0.457) & 0.04 (0.197) & 0.647 (0.478) & 0.326 (0.469) & 0.555 (0.497) \\

\midrule
\midrule
Random & 0.195 (0.396) & 0.169 (0.375) & 0.251 (0.434) & 0.167 (0.373) & 0.17 (0.375) & 0.19 (0.393) \\
\bottomrule
\end{tabular}


==> tables/images_per_dataset.tex <==
% \begin{adjustbox}{center,max width=\textwidth}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%% ADD TABLE %%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{tabular}{lp{4cm}p{6cm}llrrr}
% \label{tab:images_per_dataset}
% % \toprule
% \textbf{Dataset} & \textbf{Subdomain} & \textbf{Microscopy Submodality}  & \textbf{Images} & \textbf{Classes} & 
%  \textbf{microns/pixel} \\
% \midrule
% \textbf{Biology} \\
% Eulenberg et al 2017 & Cell and molecular biology & Darkfield, brightfield, epifluorescence & 1400x3 & 7x3& NaN \\
%   %eulenberg et al 2017 & Cell and molecular biology & Darkfield  & 6454 & 7& NaN \\
%  %eulenberg et al 2017  & Cell and molecular biology & Brightfield  & 6454 & 7& NaN \\
%  %eulenberg et al 2017  & Cell and molecular biology & Epifluorescence  & 6454 & 7& NaN \\
%  Held et al 2010 & Cell cycle & Epifluorescence  & 203 & 8 & 14.38$\times10^{-2}$  \\
%   Burgess et al 2024  & Cell biology & Synthetic & 1800 &  9& 12.5$\times10^{-2}$  \\
% % burgess et al 2024  & cell biology & Synthetic & 5400 & 3& 12.5$\times10^{-2}$  \\
 
%  %burgess et al 2024 texture & cell biology & Synthetic & 5400 & 3& 12.5$\times10^{-2}$ \\
%  %burgess et al 2024 eccentricity & cell biology & Synthetic & 5400 & 3& 12.5$\times10^{-2}$  \\
%  colocalization benchmark & Biophysics & Confocal  & 96 & 4& 5$\times10^{-2}$  \\
%  icpr2020 pollen & Botany & Brightfield  & 800 & 4& 35$\times10^{-2}$ \\
%  EMPIAR SBFSEM&  Botany, cell biology, parasitology, developmental biology, & Serial Blockface scanning electron & 587 &  5 &1.24$\times10^{-2}$  \\
%  %EMPIAR-10994 & parasitology  & serial blockface scanning electron\\
%  %EMPIAR-11464 &  & serial blockface scanning electron \\
% % EMPIAR-11831 & botany  & serial blockface scanning electron\\
% % EMPIAR-11759 &  & serial blockface scanning electron
%  \\


% \textbf{Pathology} \\
% Hussain et al 2019 & gynecologic cytology & Brightfield  & 193 & 4& 25$\times10^{-2}$  \\ 
%  Tang et al 2019 & neuropathology & Brightfield  & 800& 4& 50.3$\times10^{-2}$  \\
%  Jung et al 2022 & hematopathology & Brightfield  & 1000 & 5& 16$\times10^{-2}$  \\
%  Kather et al 2016 & gastrointestinal pathology & Brightfield  & 1000 & 8& 49.5$\times10^{-2}$  \\
% Acevedo et al 2020 & hematopathology & Brightfield  & 3419 & 8& 10$\times10^{-2}$  \\
%  Wong et al 2022 & neuropathology & Brightfield  & 800 & 4& NaN \\
%  Nirschl et al 2018 & cardiovascular pathology & Brightfield  & 400 & 2& NaN \\ 
%  \midrule
 
% \textbf{Total} &  12 &   6 & 71541 & 86 & \\
 
% \bottomrule
% \caption{Content 
% \JB{I had to comment out the `topule' command bc it caused compile error and couldnt fix it}
% }
% \end{tabular}
% \end{adjustbox}

==> tables/images_per_datasets_old.tex <==
\begin{adjustbox}{center,max width=\textwidth}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ADD TABLE %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}{lp{4cm}p{6cm}llrrr}
\toprule
\textbf{Dataset} & \textbf{Subdomain} & \textbf{Microscopy Submodality}  & \textbf{Images} & \textbf{Classes} & \textbf{microns/pixel} \\
\midrule
\textbf{Biology} \\
Eulenberg et al 2017 & Cell and molecular biology & Darkfield, brightfield, epifluorescence & 1400x3 & 7x3& NaN \\
  %eulenberg et al 2017 & Cell and molecular biology & Darkfield  & 6454 & 7& NaN \\
 %eulenberg et al 2017  & Cell and molecular biology & Brightfield  & 6454 & 7& NaN \\
 %eulenberg et al 2017  & Cell and molecular biology & Epifluorescence  & 6454 & 7& NaN \\
 Held et al 2010 & Cell cycle & Epifluorescence  & 203 & 8 & 14.38$\times10^{-2}$  \\
  Burgess et al 2024  & Cell biology & Synthetic & 1800 &  9& 12.5$\times10^{-2}$  \\
% burgess et al 2024  & cell biology & Synthetic & 5400 & 3& 12.5$\times10^{-2}$  \\
 
 %burgess et al 2024 texture & cell biology & Synthetic & 5400 & 3& 12.5$\times10^{-2}$ \\
 %burgess et al 2024 eccentricity & cell biology & Synthetic & 5400 & 3& 12.5$\times10^{-2}$  \\
 colocalization benchmark & Biophysics & Confocal  & 96 & 4& 5$\times10^{-2}$  \\
 icpr2020 pollen & Botany & Brightfield  & 800 & 4& 35$\times10^{-2}$ \\
 EMPIAR SBFSEM&  Botany, cell biology, parasitology, developmental biology, & Serial Blockface scanning electron & 587 &  5 &1.24$\times10^{-2}$  \\
 %EMPIAR-10994 & parasitology  & serial blockface scanning electron\\
 %EMPIAR-11464 &  & serial blockface scanning electron \\
% EMPIAR-11831 & botany  & serial blockface scanning electron\\
% EMPIAR-11759 &  & serial blockface scanning electron
 \\





\textbf{Pathology} \\
Hussain et al 2019 & gynecologic cytology & Brightfield  & 193 & 4& 25$\times10^{-2}$  \\ 
 Tang et al 2019 & neuropathology & Brightfield  & 800& 4& 50.3$\times10^{-2}$  \\
 Jung et al 2022 & hematopathology & Brightfield  & 1000 & 5& 16$\times10^{-2}$  \\
 Kather et al 2016 & gastrointestinal pathology & Brightfield  & 1000 & 8& 49.5$\times10^{-2}$  \\
Acevedo et al 2020 & hematopathology & Brightfield  & 3419 & 8& 10$\times10^{-2}$  \\
 Wong et al 2022 & neuropathology & Brightfield  & 800 & 4& NaN \\
 Nirschl et al 2018 & cardiovascular pathology & Brightfield  & 400 & 2& NaN \\ 
 \midrule
 
\textbf{Total} &  12 &   6 & 71541 & 86 & \\

 
\bottomrule
\end{tabular}


\end{adjustbox}

==> tables/lr.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lllllll}
\hline
Dataset & VQA, C, OD, S, Domains & Source & Images & QA Pairs & Answer type & Domains  \\
\hline
\hline
PathVQA & Pathology & PEIR Digital Library & 4,998 & 32,799 & Open & Books \\
VQA-RAD & Radiology & MedPix\textsuperscript{\textregistered} Database & 315 & 3,515 & Open/MC & 1 \\
VQAQ-Med & Radiology & MedPix\textsuperscript{\textregistered} Database & 4,200 & 15,292 & Open/MC & 1 \\
PMC-VQA & Mixture\textsuperscript{*} & PubMed Central\textsuperscript{\textregistered} & 149,000 & 227,000 & MC & \\
\dataset\ & Mixture\textsuperscript{*} &  &  & & Open/MC & \\
\hline
\hline
\end{tabular}
\caption{Comparison of  \dataset\  to existing composite  datasets (anything VQA, classification, Segmentation, but it has to be composite) check  }
\label{tab:datasets}
\end{table}

==> tables/modalities.tex <==

\begin{table*}[t]
\centering
\normalsize
\renewcommand{\arraystretch}{1.25} 
\caption{Dataset Modalities: Modalities Covered by BioMed-VLM Dataset}

\begin{center}
\begin{tabular}{ m{5em} m{2em} m{6em} m{6em} m{5em} m{5em} m{5em} m{5em} m{5em}} 
 \hline
 & &  \multicolumn{5}{c}{ \textbf{Vision (Perception) Tasks }} \\
 %\cline{2-8} 
 \hline
   & &\centering Phenotype Classification & \centering Object Detection & \centering Object Counting & \centering Cell Registration  &  \centering Semantic Segmentation & \centering Instance Segmentation & \\
 \textbf{Microscopy Modality}  &  \\ 
 \hline

 \multirow{3}{4em}{\centering Brightfield Microscopy} &  \centering PC  &  \checkmark   \\
 & \centering DIC &   \checkmark  & & & & \checkmark \\
 & \centering TL &  \\ \\

m 
 \multirow{3}{4em}{\centering Fluorescence Microscopy} &  \centering WF & \\
 & \centering CF &   \checkmark  \\
 & \centering SR  &  \\ 
 & \centering SMLM& \\

  \multirow{3}{4em}{\centering Electron Microscopy} &  \centering TEM & \\
 & \centering SEM &  \\
 & \centering ET &  \\
 
 
\end{tabular}
\end{center}
\label{tab:category_analysis}
\end{table*}


==> tables/modality_submodality_domain_subdomain_stain.tex <==
\begin{tabular}{llllllll}
\toprule
Quartile & ALIGN & BLIP & BioMedCLIP & ConchCLIP & OpenCLIP & PLIP & QuiltCLIP \\
\midrule
(37.999, 51.0] & 0.37 (0.48) & 0.2 (0.4) & 0.46 (0.5) & 0.29 (0.45) & 0.15 (0.36) & 0.17 (0.37) & 0.28 (0.45) \\
(51.0, 53.0] & 0.67 (0.47) & 0.29 (0.45) & 0.63 (0.48) & 0.11 (0.31) & 0.68 (0.47) & 0.41 (0.49) & 0.51 (0.5) \\
(53.0, 59.0] & 0.48 (0.5) & 0.2 (0.4) & 0.39 (0.49) & 0.26 (0.44) & 0.3 (0.46) & 0.47 (0.5) & 0.48 (0.5) \\
(59.0, 68.0] & 0.31 (0.46) & 0.24 (0.43) & 0.63 (0.48) & 0.14 (0.34) & 0.34 (0.47) & 0.48 (0.5) & 0.38 (0.48) \\
\bottomrule
\end{tabular}


==> tables/oldmodelparam.tex <==
\begin{table}[h]
\centering
\caption{VLM Model Breakdown:}
\label{tab:model_comparison}
\begin{adjustbox}{center,max width=\textwidth}
\begin{tabular}{lllllllll}
\toprule
\textbf{Model} & \textbf{Total Params} & \textbf{Base Model} & \textbf{Vision Encoder} & \textbf{VE Params} & \textbf{Text Encoder} & \textbf{TE Params} & \textbf{Training Data} &  Size\\
\midrule
\textbf{Contrastive VLMs} \\
ALIGN \cite{jia2021scaling} & 172.1M &&&&&& \\
BLIP \cite{li2022blip} & 223.7M \\
OpenCLIP & 223.7M & & ViT-B/32 & 86M &&& LAION-2B &34B \\
BiomedCLIP & 195.M & OpenCLIP & ViT-B/16 & 86M & BioMedBERT \cite{chakraborty2020biomedbert} & 110M & PMC-15M& 15M \\
PLIP \cite{huang2023visual} & 151.2M &&&&&& \\
CONCH \cite{lu2023towards}  & 395.2M & CoCa &&&&&& 1.17M\\
Quilt \cite{ikezogwo2024quilt} & 151.2M &&&&&& \\
OwlVIT2 & 154.9M \\
\textbf{Auto-regressive} \\
BLIP2 & 3.7B \\
CogVLM \cite{wang2023cogvlm} & 17.6B && EVA2-CLIP-E && Vicuna-1.5-7B & 7B & Multiple & 1.5B \\
Qwen-VL \cite{bai2023qwen} & 9.6B && ViT-bigG & 1.9B & QwenLM & 7.7B & Multiple &1.4B \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/pf.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|m{0.5\linewidth}|m{0.4\linewidth}|}
\hline
\multicolumn{2}{|c|}{\textbf{TASK:  White blood cell classification}} \\ 
\hline
\begin{tabular}[c]{@{}l@{}}
\textbf{Prompt:} A Giemsa-stained light micrograph displaying human peripheral blood cells. As a blood cell recognition system, identify the correct cell type: \\ \\

\textbf{Options:} \\
\textcolor{orange}{A. eosinophil}\newline B. neutrophil\newline  C. immature granulocyte\newline  D. platelet\newline  E. erythroblast\newline  F. none of the above\newline
\end{tabular} &
\vspace{3em}\includegraphics[width=\linewidth]{tables/pf0.png} \\
\hline
\end{tabular}
\end{table}

{\includegraphics[height=5em]{tables/pf0.png}} & A Giemsa-stained light micrograph displaying human peripheral blood cells. As a blood cell recognition system, identify the correct cell type: &   \textcolor{orange}{A. eosinophil}\newline B. neutrophil\newline  C. immature granulocyte\newline  D. platelet\newline  E. erythroblast\newline  F. none of the above\newline   & Giemsa stained photomicrograph of \{article\} \{class\}. & \textcolor{orange}{A. Giemsa stained photomicrograph of an eosinophil.}\newline B. Giemsa stained photomicrograph of a neutrophil.\newline  C. Giemsa stained photomicrograph of an immature granulocyte.\newline  D. Giemsa stained photomicrograph of a platelet.\newline  E. Giemsa stained photomicrograph of an erythroblast.\newline  F. none of the above\newline  \\

classification of cell contour irregularity phenotypes in synthetic images & {\includegraphics[height=5em]{tables/pf1.png}} & A synthetic fluorescence micrograph is displayed. What is the most likely description for the cell's contour irregularities? &   A. irregular\newline \textcolor{orange}{B. intermediate}\newline C. smooth\newline  D. none of the above\newline   & A micrograph acquired through \{class\}. &   A. A micrograph acquired through electron microscopy.\newline \textcolor{orange}{B. A micrograph acquired through fluorescence microscopy.}\newline C. A micrograph acquired through light microscopy.\newline  D. none of the above\newline  \\

classification of cell contour irregularity phenotypes in synthetic images & {\includegraphics[height=5em]{tables/pf2.png}} & An electron micrograph is shown. Based on the image, what is the most likely structure on the field of view? &   A. a Zebrafish retina\newline  B. Leishmania haptomonad\newline  C. a HeLa cell in metaphase\newline \textcolor{orange}{D. Cardiac muscle}\newline E. a Tobacco leaf chloroplast\newline  F. none of the above\newline    & A Serial blockface scanning electron microscopy image shows \{class\}. &    A. A Serial blockface scanning electron microscopy image shows a Zebrafish retina\newline  B. A Serial blockface scanning electron microscopy image shows Leishmania haptomonad\newline  C. A Serial blockface scanning electron microscopy image shows a HeLa cell in metaphase\newline \textcolor{orange}{D. A Serial blockface scanning electron microscopy image shows Cardiac muscle}\newline E. A Serial blockface scanning electron microscopy image shows a Tobacco leaf chloroplast\newline  F. none of the above\newline   \\

classification of cell cycle phase & {\includegraphics[height=5em]{tables/pf3.png}} & A brightfield micrograph of jurkat cells acquired using flow cytometry (single cell). Based on the micrograph, what is the most likely cell phase? &   A. interphase (G2)\newline \textcolor{orange}{B. interphase (G1) phase}\newline C. Telophase\newline  D. Anaphase\newline  E. Synthesis\newline  F. none of the above\newline & A Brightfield microscopy imaging flow cytometry is used to visualize single Jurkat cells at different cell cycle phases. The image displays a cell in \{class\} stage of the cell cycle. &    A. Brightfield microscopy imaging flow cytometry is used to visualize single Jurkat cells at different cell cycle phases. The image displays a cell in interphase (G2) stage of the cell cycle.\newline \textcolor{orange}{B. Brightfield microscopy imaging flow cytometry is used to visualize single Jurkat cells at different cell cycle phases. The image displays a cell in interphase (G1) phase stage of the cell cycle.}\newline C. Brightfield microscopy imaging flow cytometry is used to visualize single Jurkat cells at different cell cycle phases. The image displays a cell in Telophase stage of the cell cycle.\newline  D. Brightfield microscopy imaging flow cytometry is used to visualize single Jurkat cells at different cell cycle phases. The image displays a cell in Anaphase stage of the cell cycle.\newline  E. Brightfield microscopy imaging flow cytometry is used to visualize single Jurkat cells at different cell cycle phases. The image displays a cell in Synthesis stage of the cell cycle.\newline  F. none of the above\newline  \\

classification of cell cycle stages in live cell imaging data & {\includegraphics[height=5em]{tables/pf4.png}} & A fluorescence micrograph of Hela Kyoto cells stably expressing GalT-eGFP to label the Golgi apparatus. Based on the image what is the most likely the Golgi apparatus morphology? &    A. Anaphase\newline  B. Diffuse\newline \textcolor{orange}{C. Interphase}\newline D. Golgi twin\newline  E. Partly disassembled\newline  F. none of the above\newline  & "Fluorescence microscopy image of human Hela Kyoto cells stably expressing galactosyltransferase (GalT-eGFP) to label the Golgi apparatus showing \{class\} morphology. &    A. Fluorescence microscopy image of human Hela Kyoto cells stably expressing galactosyltransferase (GalT-eGFP) to label the Golgi apparatus showing Anaphase morphology.\newline  B. Fluorescence microscopy image of human Hela Kyoto cells stably expressing galactosyltransferase (GalT-eGFP) to label the Golgi apparatus showing Diffuse morphology.\newline \textcolor{orange}{C. Fluorescence microscopy image of human Hela Kyoto cells stably expressing galactosyltransferase (GalT-eGFP) to label the Golgi apparatus showing Interphase morphology.}\newline D. Fluorescence microscopy image of human Hela Kyoto cells stably expressing galactosyltransferase (GalT-eGFP) to label the Golgi apparatus showing Golgi twin morphology.\newline  E. Fluorescence microscopy image of human Hela Kyoto cells stably expressing galactosyltransferase (GalT-eGFP) to label the Golgi apparatus showing Partly disassembled morphology.\newline  F. none of the above\newline \\

Classification of pre-cancerous and cervical cancer lesions in liquid-based cytology Pap smear images & {\includegraphics[height=5em]{tables/pf5.png}} & Liquid-based cytology pap smear of human pre-cancerous or cervical cancer lesions. Based on the cytogram, what is the most likely finding? &    A. Squamous cell carcinoma (SCC)\newline  B. Low-grade (LSIL)\newline \textcolor{orange}{C. Negative (NILM)}\newline D. High-grade (HSIL)\newline  E. none of the above\newline & Liquid-based cytology Pap smear reveals the presence of \{class\} lesions.&     A. Liquid-based cytology Pap smear reveals the presence of Squamous cell carcinoma (SCC) lesions.\newline  B. Liquid-based cytology Pap smear reveals the presence of Low-grade (LSIL) lesions.\newline \textcolor{orange}{C. Liquid-based cytology Pap smear reveals the presence of Negative (NILM) lesions.}\newline D. Liquid-based cytology Pap smear reveals the presence of High-grade (HSIL) lesions.\newline  E. none of the above\newline \\

classification of normal and abnormal pollen grains & {\includegraphics[height=5em]{tables/pf6.png}} & Basic fuchsin stained light micrograph of pollen grains. Based on the image, what is the most likely pollen class? &     A. abnormal Corylus avellana\newline \textcolor{orange}{B. Non-pollen}\newline C. normal Alnus\newline  D. normal Corylus avellana\newline  E. none of the above\newline & A brightfield microscopy image of pollen grains shows \{class\} structures. &      A. A brightfield microscopy image of pollen grains shows abnormal Corylus avellana structures.\newline \textcolor{orange}{B. A brightfield microscopy image of pollen grains shows Non-pollen structures.}\newline C. A brightfield microscopy image of pollen grains shows normal Alnus structures.\newline  D. A brightfield microscopy image of pollen grains shows normal Corylus avellana structures.\newline  E. none of the above\newline \\

white blood cell classification (jung) & {\includegraphics[height=5em]{tables/pf7.png}} & Synthetically generated Giemsa-stained light micrograph of human peripheral blood cell. As a blood cell recognition system, identify the correct cell type: &   \textcolor{orange}{A. Neutrophil}\newline B. Basophil\newline  C. Lymphocyte\newline  D. Eosinophil\newline  E. Monocyte\newline  F. none of the above\newline   & A synthetic microscopy image of a peripheral blood smear stained with giemsa, displays \{article\} \{class\}. &  \textcolor{orange}{A. A synthetic microscopy image of a peripheral blood smear stained with giemsa, displays a Neutrophil.}\newline B. A synthetic microscopy image of a peripheral blood smear stained with giemsa, displays a Basophil.\newline  C. A synthetic microscopy image of a peripheral blood smear stained with giemsa, displays a Lymphocyte.\newline  D. A synthetic microscopy image of a peripheral blood smear stained with giemsa, displays an Eosinophil.\newline  E. A synthetic microscopy image of a peripheral blood smear stained with giemsa, displays a Monocyte.\newline  F. none of the above\newline \\

texture classification in colorectal cancer & {\includegraphics[height=5em]{tables/pf8.png}} & H\&E stained light micrograph of human colorectal tissue. Based on the image, what is the most likely texture class? &   A. chronic heart failure\newline \textcolor{orange}{B. not chronic heart failure}\newline C. none of the above\newline   & H\&E stained light microscopy image of human cardiac tissue with \{class\} texture. &  A. H\&E stained light microscopy image of human colorectal tissue with debris and mucus.\newline \textcolor{orange}{B. H\&E stained light microscopy image of human colorectal tissue with complex stroma (with single tumor or immune cells).}\newline C. H\&E stained light microscopy image of human colorectal tissue with mucosal glands.\newline  D. H\&E stained light microscopy image of human colorectal tissue with background.\newline  E. H\&E stained light microscopy image of human colorectal tissue with simple stroma.\newline  F. none of the above\newline  \\

classification of heart failure using cardiac histopathology images & {\includegraphics[height=5em]{tables/pf9.png}} & H\&E stained light micrograph of human cardiac tissue. Based on the image, what is the most likely clinical chronic heart diagnosis? &  A. chronic heart failure\newline \textcolor{orange}{B. not chronic heart failure}\newline C. none of the above\newline & H\&E stained light microscopy image of human cardiac tissue with {class} texture.&  A. H\&E stained light microscopy image of human cardiac tissue with chronic heart failure texture.\newline \textcolor{orange}{B. H\&E stained light microscopy image of human cardiac tissue with not chronic heart failure texture.}\newline C. none of the above\newline\\

amyloid beta pathology classification & {\includegraphics[height=5em]{tables/pf10.png}} & IHC stained light micrograph of extracellular amyloid-beta deposition in the human brain tissue. Based on the image, what is the most likely amyloid beta morphology pattern? &  A. cerebral amyloid angiopathy\newline \textcolor{orange}{B. diffuse plaque}\newline C. cored plaque\newline  D. negative\newline  E. none of the above\newline  & Human brain tissue is stained with immunohistochemistry for amyloid-beta and imaged using brightfield microscopy. The micrograph displays \{class\} patterns. &  A. Human brain tissue is stained with immunohistochemistry for amyloid-beta and imaged using brightfield microscopy. The micrograph displays cerebral amyloid angiopathy patterns.\newline \textcolor{orange}{B. Human brain tissue is stained with immunohistochemistry for amyloid-beta and imaged using brightfield microscopy. The micrograph displays diffuse plaque patterns.}\newline C. Human brain tissue is stained with immunohistochemistry for amyloid-beta and imaged using brightfield microscopy. The micrograph displays cored plaque patterns.\newline  D. Human brain tissue is stained with immunohistochemistry for amyloid-beta and imaged using brightfield microscopy. The micrograph displays negative patterns.\newline  E. none of the above\newline  \\

amyloid beta pathology classification & {\includegraphics[height=5em]{tables/pf11.png}} & IHC stained light micrograph of extracellular amyloid-beta deposition in the human brain tissue. Based on the image, what is the most likely amyloid beta morphology pattern? &  A. Caa\newline  B. Cored\newline \textcolor{orange}{C. Negative}\newline D. Diffuse\newline  E. none of the above\newline  & Human brain tissue is stained with immunohistochemistry for amyloid-beta and imaged using brightfield microscopy. The micrograph displays {class} patterns. &  A. Human brain tissue is stained with immunohistochemistry for amyloid-beta and imaged using brightfield microscopy. The micrograph displays Caa patterns.\newline  B. Human brain tissue is stained with immunohistochemistry for amyloid-beta and imaged using brightfield microscopy. The micrograph displays Cored patterns.\newline \textcolor{orange}{C. Human brain tissue is stained with immunohistochemistry for amyloid-beta and imaged using brightfield microscopy. The micrograph displays Negative patterns.}\newline D. Human brain tissue is stained with immunohistochemistry for amyloid-beta and imaged using brightfield microscopy. The micrograph displays Diffuse patterns.\newline  E. none of the above\newline  \\

classification of mitochondrial morphology in CryoET images & {\includegraphics[height=5em]{tables/pf12.png}} & A cryo-electron tomography of mitochondria in neurons cultured in vitro is shown. Based on the image what is the most likely mitochondrial morphology? &  A. abnormal mitochondrial morphology\newline \textcolor{orange}{B. normal mitochondrial morphology}\newline C. none of the above\newline  & A cryo-electron tomography of mitochondria in neurons cultured in vitro shows \{class\}. &  A. A cryo-electron tomography of mitochondria in neurons cultured in vitro shows abnormal mitochondrial morphology.\newline \textcolor{orange}{B. A cryo-electron tomography of mitochondria in neurons cultured in vitro shows normal mitochondrial morphology.}\newline C. none of the above\newline  \\

\hline
\caption{\textbf{Examples of fine-grained perception dataset.} Each example has a user-inputted image and question pair. There are four multiple choice answers for each question (correct choice highlighted in \textcolor{orange}{orange}).}
\end{longtable}

==> tables/scales.tex <==

\begin{table}[h!]
\centering
\caption{Overview of biological length scales, modalities, and structures}
\begin{tabular}{p{1.5cm}p{4cm}p{5cm}p{1.4cm}p{1.4cm}}
\toprule
\textbf{Scale} & \textbf{Modality} & \textbf{Biological structures} & \textbf{Lower Range} & \textbf{Upper Range} \\ 
\midrule
Nanometer  & Electron microscopy, Super-resolution microscopy & Viruses, molecules, DNA and protein microstructure, organelle microstructure & 0.25 nm & 250 nm \\ 
Micrometer & Fluorescence microscopy, Brightfield microscopy & Proteins, organelle macrostructure, bacteria, cell microstructure, tissue microstructure & 0.25 µm (250 nm) & 250 µm (0.1 mm) \\
Macrometer  & Fluorescence microscopy, Brightfield microscopy, Dissecting microscope & Cell macrostructure, tissues & 0.25 mm (250 µm) & 25 mm (2.5 cm) \\ \bottomrule
\end{tabular}
\label{table:biological_length_scales}
\end{table}

